A random Hall-Paige conjecture

A complete mapping of a group $G$ is a bijection $\phi\colon G\to G$ such that $x\mapsto x\phi(x)$ is also bijective. Hall and Paige conjectured in 1955 that a finite group $G$ has a complete mapping whenever $\prod_{x\in G} x$ is the identity in the abelianization of $G$. This was confirmed in 2009 by Wilcox, Evans, and Bray with a proof using the classification of finite simple groups. \par In this paper, we give a combinatorial proof of a far-reaching generalisation of the Hall-Paige conjecture for large groups. We show that for random-like and equal-sized subsets $A,B,C$ of a group $G$, there exists a bijection $\phi\colon A\to B$ such that $x\mapsto x\phi(x)$ is a bijection from $A$ to $C$ whenever $\prod_{a\in A} a \prod_{b\in B} b=\prod_{c\in C} c$ in the abelianization of $G$. We use this statement as a black-box to settle the following old problems in combinatorial group theory for large groups. (1) We characterise sequenceable groups, that is, groups which admit a permutation $\pi$ of their elements such that the partial products $\pi_1$, $\pi_1\pi_2$, $\pi_1\pi_2\cdots \pi_n$ are all distinct. This resolves a problem of Gordon from 1961 and confirms conjectures made by several authors, including Keedwell's 1981 conjecture that all large non-abelian groups are sequenceable. We also characterise the related $R$-sequenceable groups, addressing a problem of Ringel from 1974. (2) We confirm in a strong form a conjecture of Snevily from 1999 by characterising large subsquares of multiplication tables of finite groups that admit transversals. Previously, this characterisation was known only for abelian groups of odd order (by a combination of papers by Alon and Dasgupta-K\'arolyi-Serra-Szegedy and Arsovski).

==> table3absorber.tex <==
 \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
 & $u$ & $w$ & $w^{-1}b^{-1}$ & $w^{-1}d^{-1}$ & $a^{-1}u^{-1}$ & $c^{-1}u^{-1}$ & $bwua$ & $dwuc$ \\ \hline
$u$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{D9E1F2}$a$ & \cellcolor[HTML]{D9E1F2}$c$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ \\ \hline
$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{D9E1F2}$d$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ \\ \hline
$w^{-1}b^{-1}$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$d^{-1}b$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ \\ \hline
$w^{-1}d^{-1}$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{D9E1F2}$d$ & \cellcolor[HTML]{FFF2CC}$d^{-1}b$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ \\ \hline
$a^{-1}u^{-1}$ & \cellcolor[HTML]{D9E1F2}$a$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$ac^{-1}$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ \\ \hline
$c^{-1}u^{-1}$ & \cellcolor[HTML]{D9E1F2}$c$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{FFF2CC}$ac^{-1}$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ \\ \hline
$bwua$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9} \\ \hline
$dwuc$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9} \\ \hline
\end{tabular}


==> tablecleancommutator.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
 & $u$ & $w^{-1}$ & $z^{-1}x^{-1}u^{-1}$ & $z^{-1}[b,a]x^{-1}u^{-1}$ & $uxzw$ & $ux[a,b]zw$ \\ \hline
$u$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{D9E1F2}$xz$ & \cellcolor[HTML]{D9E1F2}$x[a,b]z$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ \\ \hline
$w^{-1}$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$u$ \\ \hline
$z^{-1}x^{-1}u^{-1}$ & \cellcolor[HTML]{D9E1F2}$xz$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFE699}$[b,a]$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ \\ \hline
$z^{-1}[b,a]x^{-1}u^{-1}$ & \cellcolor[HTML]{D9E1F2}$x[a,b]z$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{FFE699}$[b,a]$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ \\ \hline
$uxzw$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFE699}$[a,b]$ \\ \hline
$ux[a,b]zw$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$u$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{E2EFDA}$w$ & \cellcolor[HTML]{FFE699}$[a,b]$ & \cellcolor[HTML]{D9D9D9} \\ \hline
\end{tabular} 

==> tablecommutator.tex <==
 \begin{landscape}
\begin{figure}[h]
\tiny											
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
 &	\rotatebox{90}{$\hat z^{-1}$}	&	\rotatebox{90}{$\hat z^{-1}z^{-1}$}	&	\rotatebox{90}{$\hat b$}	&	\rotatebox{90}{$\hat b b$}	&	\rotatebox{90}{$\hat a$}	&	\rotatebox{90}{$\hat a a$}	&	\rotatebox{90}{$z^{-1}x^{-1}v^{-1}$}	&	\rotatebox{90}{$z^{-1}[b,a]x^{-1}v^{-1}$}	&	\rotatebox{90}{$[b,a]x^{-1}v^{-1}$}	&	\rotatebox{90}{$ab^{-1}a^{-1}x^{-1}v^{-1}$}	&	\rotatebox{90}{$b^{-1}a^{-1}x^{-1}v^{-1}$}	&	\rotatebox{90}{$a^{-1}x^{-1}v^{-1}$}	&	\rotatebox{90}{$x^{-1}v^{-1}$}	&	\rotatebox{90}{$vxz \hat z$}	&	\rotatebox{90}{$v$}	&	\rotatebox{90}{$vx[a,b]z \hat z$}	&	\rotatebox{90}{$vxaba^{-1}b^{-1}\hat b^{-1}$}	&	\rotatebox{90}{$vxaba^{-1}\hat a^{-1}$}	&	\rotatebox{90}{$vxa\hat b^{-1}$}	&	\rotatebox{90}{$vx\hat a^{-1}$}\\ \hline
$\hat z^{-1}$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ \\ \hline
$\hat   z^{-1}z^{-1}$ & \cellcolor[HTML]{FFF2CC}$z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ \\ \hline
$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ \\ \hline
$\hat b b$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{FFF2CC}$b$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ \\ \hline
$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ \\ \hline
$\hat a a$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{FFF2CC}$a$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ \\ \hline
$z^{-1}x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$[b,a]$ & \cellcolor[HTML]{FFF2CC}$z[b,a]$ & \cellcolor[HTML]{FFF2CC}$zab^{-1}a^{-1}$ & \cellcolor[HTML]{FFF2CC}$zb^{-1}a^{-1}$ & \cellcolor[HTML]{FFF2CC}$za^{-1}$ & \cellcolor[HTML]{FFF2CC}$z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$xz$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$z^{-1}[b,a]x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$[b,a]$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$z$ & \cellcolor[HTML]{FFF2CC}$zb$ & \cellcolor[HTML]{FFF2CC}$zba$ & \cellcolor[HTML]{FFF2CC}$zbab^{-1}$ & \cellcolor[HTML]{FFF2CC}$z[a,b]$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$x[a,b]z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$[b,a]x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$z[b,a]$ & \cellcolor[HTML]{FFF2CC}$z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$a$ & \cellcolor[HTML]{FFF2CC}$ba$ & \cellcolor[HTML]{FFF2CC}$bab^{-1}$ & \cellcolor[HTML]{FFF2CC}$[b,a]$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$x[a,b]$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$ab^{-1}a^{-1}x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$zab^{-1}a^{-1}$ & \cellcolor[HTML]{FFF2CC}$zb$ & \cellcolor[HTML]{FFF2CC}$a$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$a$ & \cellcolor[HTML]{FFF2CC}$ab^{-1}$ & \cellcolor[HTML]{FFF2CC}$ab^{-1}a^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$xaba^-1$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$b^{-1}a^{-1}x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$zb^{-1}a^{-1}$ & \cellcolor[HTML]{FFF2CC}$zba$ & \cellcolor[HTML]{FFF2CC}$ba$ & \cellcolor[HTML]{FFF2CC}$a$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$b^{-1}$ & \cellcolor[HTML]{FFF2CC}$b^{-1}a^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$xab$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$a^{-1}x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$za^{-1}$ & \cellcolor[HTML]{FFF2CC}$zbab^{-1}$ & \cellcolor[HTML]{FFF2CC}$bab^{-1}$ & \cellcolor[HTML]{FFF2CC}$ab^{-1}$ & \cellcolor[HTML]{FFF2CC}$b^{-1}$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{FFF2CC}$a^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$xa$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$x^{-1}v^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$z$ & \cellcolor[HTML]{FFF2CC}$z[a,b]$ & \cellcolor[HTML]{FFF2CC}$[b,a]$ & \cellcolor[HTML]{FFF2CC}$ab^{-1}a^{-1}$ & \cellcolor[HTML]{FFF2CC}$b^{-1}a^{-1}$ & \cellcolor[HTML]{FFF2CC}$a^{-1}$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9E1F2}$x$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$vxz \hat z$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{FFF2CC}$[a,b]$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{D9E1F2}$xz$ & \cellcolor[HTML]{D9E1F2}$x[a,b]z$ & \cellcolor[HTML]{D9E1F2}$x[a,b]$ & \cellcolor[HTML]{D9E1F2}$xaba^-1$ & \cellcolor[HTML]{D9E1F2}$xab$ & \cellcolor[HTML]{D9E1F2}$xa$ & \cellcolor[HTML]{D9E1F2}$x$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat a$ \\ \hline
$vx[a,b]z   \hat z$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{FFF2CC}$[a,b]$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat z$ \\ \hline
$vxaba^{-1}b^{-1}\hat   b^{-1}$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{FFF2CC}$ba^{-1}b^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat b$ \\ \hline
$vxaba^{-1}\hat   a^{-1}$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{FFF2CC}$aba^{-1}$ \\ \hline
$vxa\hat   b^{-1}$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{FFF2CC}$ba^{-1}b^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{E2EFDA}$\hat b$ \\ \hline
$vx\hat a^{-1}$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$v$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat a$ & \cellcolor[HTML]{E2EFDA}$\hat z$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{FFF2CC}$aba^{-1}$ & \cellcolor[HTML]{E2EFDA}$\hat b$ & \cellcolor[HTML]{D9D9D9} \\ \hline
\end{tabular}														
  \caption{Justification for all pairs of words in $R'$ being separable. The $(i,j)$th entry explains why the equation $i=j$ is of one of the types in the definition of ``separable''. The three colours correspond to the three types of equations in the definition with white corresponding to type 1, blue to type 2, and orange to type 3. The variables in the white cells are a variable which occurs in one of the words $i$/$j$, but not both. For the blue cells, the equations $i=j$ rearrange into $(v^{-1})^2=g$  where $g$ is the entry in the cell. For the orange cells the equations rearrange into $g=\id$ where $g$ is the entry in the cell. }
\label{Figure_justification_commutator}
\end{figure} 
  \end{landscape}												
